HALC: Object Hallucination Reduction via Adaptive Focal-Contrast Decoding

While large vision-language models (LVLMs) have demonstrated impressive capabilities in interpreting multi-modal contexts, they invariably suffer from object hallucinations (OH). We introduce HALC, a novel decoding algorithm designed to mitigate OH in LVLMs. HALC leverages distinct fine-grained optimal visual information in vision-language tasks and operates on both local and global contexts simultaneously. Specifically, HALC integrates a robust auto-focal grounding mechanism (locally) to correct hallucinated tokens on the fly, and a specialized beam search algorithm (globally) to significantly reduce OH while preserving text generation quality. Additionally, HALC can be integrated into any LVLMs as a plug-and-play module without extra training. Extensive experimental studies demonstrate the effectiveness of HALC in reducing OH, outperforming state-of-the-arts across four benchmarks.

==> content/method.tex <==
\section{Methodology}\label{sec:method}
In this section, we outline the proposed HALC from four aspects. 
%
First, we begin by examining existing 
analysis~\cite{biten2022let, zhou2023analyzing, leng2023mitigating, huang2023opera} 
to support our key hypothesis that OH primarily results from visual priors being 
under-utilized.
%
Then we provide an empirical analysis to illustrate the important relationship between 
OH and visual priors that have different visual context windows (i.e., field-of-views 
(FOVs)), and showcase the effectiveness of an optimal visual prior in correcting 
hallucination. 
%
Thirdly, building upon the observation that a more precise choice of visual priors is 
crucial to reducing OH, we propose HALC, a novel sampling-based decoding algorithm 
that mitigates OH by approximating optimal visual prior in the discretized FOV space.
%
After identifying top $k$ best proxies based on OH distribution pattern 
(\figref{fig:optimal_visual_prior}), we contrast among different pairs of FOVs to 
amplify the unique representation in each visual field~\cite{li2022contrastive}. 
%
Finally, HALC adopts a matching-based beam search algorithm with visual-response similarity as 
the beam score to ensure uncompromised linguistic qualities besides reducing 
hallucinations, a topic that is often less attended in previous 
studies~\cite{huang2023opera, leng2023mitigating}.
%
An overview of the proposed HALC is shown in \figref{fig:halc_overview}.
%
 
%A more in-depth explanation of this optimization strategy is provided in Section~\ref{subsec:beam_search}.
%
%Combining both components, an overview of the proposed HALC is showed in Figure.~\ref{fig:halc_overview}.


%In this section, we outline the proposed HALC from four aspects. First, we begin by examining existing analysis~\cite{biten2022let, zhou2023analyzing, leng2023mitigating, huang2023opera} to support our key hypothesis that OH primarily result from visual priors being under-utilized. Then we provide 
%
%We begin by examining existing analysis~\cite{biten2022let, zhou2023analyzing, leng2023mitigating, huang2023opera} to support our key hypothesis that OH primarily result from visual priors being under-utilized.
%
%More specifically, we believe that such imbalance which favors textual over visual information inherits from the auto-regressive nature of modern LVLMs.
%
%Therefore, it is a non-trivial task to correct and requires more thoughtful solutions.
%
%We extend this discussion in Section~\ref{subsec:oh_origin}.
%

%Next, we illustrate an important relationship between OH and visual priors that have 
%different visual context windows, i.e., field-of-views (FOVs).
%
% The relationship is 
%
%Specifically, we notice that the majority of object existence, attribute and relationship hallucinations can be effectively mitigated by decoding with the most appropriate visual priors.
%
%We explore this relationship with more details in Section~\ref{subsec:relationship}.
%

% Building upon the relationship where more precised uses of visual priors are crucial to reducing OH, we develop HALC, a novel decoding algorithm that aims to mitigate OH through optimal visual prior approximation.
%

%HALC is consist of two components, a local token correction process,\textit{adaptive focal-contrast grounding}, that corrects the hallucinating token with the near-optimal visual prior approximated through adaptive contrast.
%
%We illustrate this algorithm in Section~\ref{subsec:focal_contrast_grounding}.
%

%To ensure uncompromised linguistic quality while reducing OH, a topic that is often less attended in recent studies~\cite{huang2023opera, leng2023mitigating}, the second component of HALC is a uniquely designed \textit{matching-based beam search} optimization that uses visual-response similarity as beam score to seemingly ensure qualities besides reducing hallucinations.
%
%A more in-depth explanation of this optimization strategy is provided in Section~\ref{subsec:beam_search}.
%
%Combining both components, an overview of the proposed HALC is showed in Figure.~\ref{fig:halc_overview}.

\subsection{Problem Statement}\label{sec:problem}
For an LVLM $\mathcal{M}_\theta^{\text{LVLM}}$ parametrized by $\theta$, a visual encoder $\phi$ is employed to convert 
the input image into an embedding, which is then projected into the input space of a 
language model decoder through a multi-modal projection layer. 
%
Given a textual query $x$ and a visual input $v$, the model auto-regressively generate 
a response $y$ based on probability distribution $p_{\theta}(y_t | v, x, y_{<t})$. 
%
Mathematically, we have
%
% \begin{align}
% y_t &\sim p_{\theta}(y_t | v, x, y_{<t}), \\
% &\propto \exp \text{logit}_{\theta}(y_t | v, x, y_{<t}) \nonumber
% \end{align}
\begin{equation}
y_t \sim p_{\theta}(y_t | v, x, y_{<t}) \propto \exp \text{logit}_{\theta}(y_t | v, x, y_{<t})
\end{equation}
%
where $y_t$ denotes the $t^{th}$ token, and $y_{<t}$ represents the token sequence  generated up to time step $t$. 
%
The goal of HALC is to minimize the occurrence of hallucination tokens and preserve the truthfulness to both $x$ and $v$, while maintaining a high-quality linguistic flow in response $y$.
%

In Section~\ref{subsec:oh_origin}, we show that OH primarily results from visual priors being under-utilized. 
%
Conversely, we posit that there exists an optimal visual prior \jz{how do people use the term} $v^*$ capable of 
delivering the most relevant context for safely decoding each token. \jz{note to myself: a bit more clarity}
%


\subsection{Under-Utilized Visual Prior}\label{subsec:oh_origin}
OH in VLMs can be attributed to various factors, including but not limited to the 
inherent biases in the training data caused by 
co-occurrence~\cite{biten2022let, zhou2023analyzing}, visual 
uncertainty due to model's statistical bias and priors~\cite{leng2023mitigating}, as
well as the limitations in current models' ability to discern context and fact
accurately during the entire output generation process~\cite{daunhawer2021limitations}.
%
Studies have also shown that OH is not random but exhibits certain
patterns and dependencies, such as their co-existence with knowledge aggregation 
pattern~\cite{huang2023opera}, and the tendency to occur with objects positioned later
in the generated descriptions~\cite{zhou2023analyzing}.
%

A closer examination of these analysis suggests that the auto-regressive nature of the
LVLMs may just be the fundamental factor contributing to their hallucinatory behaviors.
%
Specifically, auto-regressive decoding makes LVLMs progressively rely more on 
textual priors including both textual input and the generated tokens, while unavoidably 
reducing reliance on the visual prior.
%
This imbalance results in a significant deviation from accurate representation of the
visual input, and ultimately culminating in OH with behaviors and patterns 
observed in the aforementioned existing 
studies~\cite{zhou2023analyzing, leng2023mitigating}.
%
This is especially obvious in the case when longer responses are generated, which 
explains the correlation between higher OH and larger maximum token lengths, 
as seen in~\cite{huang2023opera}.
%
\jz{this section is great in content, but maybe not in the good place? more of background or motivation than the actual method. we could split it up more clearly}

\subsection{Optimal Visual Prior for Decoding}\label{subsec:relationship}
While constantly \textit{reminding} the visual prior during the decoding process could 
mitigate the disproportionate emphasis on the textual and visual priors, it is a 
non-trivial task since simply inserting the visual prior into the middle of the 
generation is contradictory to LVLMs' causal modeling objectives~\cite{min2023recent}, 
which could degrade the flow of the generated sentences and make the output unreadable.
%

On the other hand, an alternative is to have more fine-grained control on retrieving 
the optimal visual prior for each token being generated.
%
Therefore, inspired by the success of (textual) prompt engineering in improving LLM 
responses~\cite{chen2023unleashing}, our key insight in mitigating OH lies in 
identifying a token-wise optimal visual prior to provide the most informative 
visual grounding while decoding this specific token.
%
\begin{figure}[t]
    \centering
    \includegraphics[width=0.5\textwidth]{figures/visual_priors_v2.pdf}
    \caption{
    By leveraging optimal visual priors, in average over 84.5\% of the observed 
    existence attribute, and relationship hallucinations are eliminated.
    }
    \label{fig:pattern_analysis}
    \vspace{-0.15in}
\end{figure}
%

We verify our hypothesis through empirical studies, where we showcase the performance 
of optimal visual priors in correcting the three major aforementioned sources of 
hallucination based on the MME benchmark~\cite{fu2023mme}. 
%
As shown in Figure~\ref{fig:pattern_analysis}, we see that for most cases, 
there exists an optimal visual prior where decoding from it eliminates 
over 84.5\% of the hallucinations.
%
More details on how we conducted the analysis are illustrated in 
Appendix~\ref{app:priors}.
\jz{we probably need a bit more clarity here, such as describing the procedure of the analysis, to make this example better understood and convincing as to justify the motivation.}
%

However, directly retrieving such optimal visual prior is intractable in practice.
%
Therefore, we propose to approximate the resulting logits distribution of the optimal 
visual prior through adaptive focal-contrast grounding, which will be illustrated in section~\ref{subsec:focal_contrast_grounding}.
%

\jz{the above is also not part of the method. we could probably split it up to background, or motivation section dedicated to the visual prior under-utilized issue}

\subsection{Adaptive Focal-Contrast Grounding}\label{subsec:focal_contrast_grounding}

\jz{methods start here.}

In this section, we introduce the \textit{adaptive focal-contrast grounding} module, 
whose goal is to approximate the logits distribution decoded from the optimal visual 
prior \jz{we'd better define it a bit more explicitly in previous sections to make it less like made up} and then correct the hallucinating token to maintain a healthy flow \jz{"healthy" sounds a bit informal} for the 
subsequent auto-regressive decoding.
%
%so that OH is eliminated from the token level.
% %
% The corrected token will then replace the original (hallucinating) token in the current 
% response for the subsequent auto-regressive decoding.
%

Adaptive focal-contrast grounding consists of three components: 
(1) token filtering, which identifies tokens that may linguistically 
 may contribute to object existence, attribute and/or relationship hallucination; 
(2) visual prior grounding, which locates the area in the visual prior that corresponds to the current hallucinating token;
and (3) logits redistribution, which re-weighs the logits probabilities to amplify 
the near-optimal visual priors retrieved from contrasted FOVs.
%

\paragraph{Token filtering.}
%While adaptive focal-contrast grounding can be applied to all the tokens generated by the conventional decoding, it comes at the cost of wasting tremendous run time and computational resources on irrelevant words, including determiners such as "a", "the", "every", and conjunctions such as "and", "or", "because".
%
To focus on most-probable hallucination sources and optimize 
time efficiency, we adopt part-of-speech (POS) tagging~\cite{honnibal2017spacy} to 
selectively filter in noun, adjective/adverb/number/verb/pronoun, and preposition, 
which correspond to the existence, attribute, and relationship hallucinations 
respectively.
%
%Therefore, when a new token is generated, we first identify its type by part-of-speech (POS) tagging~\cite{honnibal2017spacy} and only keep tokens belonging to noun, adjective/adverb/number/verb/pronoun, and preposition, which correspond to the existence, attribute, and relationship hallucinations respectively.
%
For example in Figure~\ref{fig:halc_overview}, the newly generated token 
\textit{surfboard} passes the filtering process as it may contribute to the object 
\textit{existence} hallucination.
%

\paragraph{Visual prior grounding.}
Next, we proceed to retrieve the visual grounding $v_d$ for the hallucinating token.
%
Specifically, we employ zero-shot detectors $\mathcal{G}_{d}$ such as Grounding DINO~\cite{liu2023grounding}, 
or OWLv2~\cite{minderer2023scaling} to locate the token in the input image.
%

Interestingly, our findings reveal that although the hallucinating token is technically 
non-existent (e.g., \textit{surfboard} in figure~\ref{fig:halc_overview}), it can still 
be accurately located by the detector in practice. 
%
This suggests that OH stems from more non-trivial causes than previously identified 
biases such as textual co-occurrence. 
%
Moreover, this source of hallucination often proves invariant to the visual encoder and 
can leads to failures of various visual perception models.
%

% One interesting finding is that, although the token that we are locating technically does not 
% exist in the visual prior as it is an hallucination, such as the "surfboard" in 
% figure~\ref{fig:halc_overview}, in practice it can still be located accurately by the detector.
% %
% This implicitly indicates that OH is a non-trivial consequence caused by more complex reasons
% than the discovered bias such as textual co-occurrence, but the more in-depth exploration in this 
% direction is outside the scope of this paper.
% %

Notably, despite the most common use case of these zero-shot detectors 
is to locate objects, they are trained to also provide good visual reference for 
adjective or prepositional phrase.
%
Because during pre-training, the objective of these detection models is to associate 
words in text descriptions with specific regions in images~\cite{liu2023grounding}, 
which naturally includes attributes and relationships.
%

\paragraph{Logits redistribution.}\label{para:logits_redistribution}
\begin{figure}[t]
    \centering
    \includegraphics[width=0.5\textwidth]{figures/teaser_v4.pdf}
    \caption{
    Likelihood of object tokens w.r.t. visual prior samples in the FOV space. Exponential 
    sampling distribution is adopted in this example. 
    %
    While obvious objects (e.g. \textit{beach}, \textit{man}) are stable with high 
    likelihood, hallucinating objects are either noisy (e.g. \textit{book}) or shift 
    gradually with the context (e.g. \textit{surfboard}). 
    %
    The victim token (e.g. \textit{clock}) usually display a drastically peaking pattern (local maximum).
    }\label{fig:optimal_visual_prior}
    \vspace{-0.15in}
\end{figure}
%
While grounding establishes a meaningful reference within the original image input, it 
often is not directly the optimal visual prior for decoding, %\rv{and directly using $\tilde{v}_d$ as a proxy for $v^*$ is highly unstable and could still result in hallucination, as shown in Figure~\ref{fig:optimal_visual_prior}}.
and directly using $\tilde{v}_d$ as a proxy for $v^*$ is highly unstable and could still result in hallucination, as shown in Figure~\ref{fig:optimal_visual_prior}.
%
% For example in figure~\ref{fig:optimal_visual_prior}, the peak that indicates highest probability for
% the correct token \textit{clock} does not happen with the grounded region returned by the detector.
%
% , we try
% to approximate the logits distribution that would have been the decoding result from 
% this unknown optimal prior.
%
Since directly retrieving such optimal visual prior from the image is intractable, we 
propose to approximate the resulting logits distribution of the optimal visual prior by 
sampling from the discretized FOV space. 
%
Specifically, let $\pi_{f}$ be an arbitrary sampling distribution, we sample $n$ FOVs 
conditioned on the initial grounding $\tilde{v}_d$:%, that is:
%
\begin{equation}\label{eqn:FoV_sample}
    \{\tilde{v}_1, \tilde{v}_2, \ldots, \tilde{v}_n\} \sim \pi_{f}(\tilde{v} | \tilde{v}_d), \quad \pi_{f} \in \Omega
\end{equation}
%
where $\Omega$ denotes the sampling space over all potential visual priors. 
%
Then we feed these sampled priors back into the LVLM and obtain $n$ corresponding 
logits distributions.
%
% We argue that such problem statement is in fact more aligned with our end goal, while 
% building upon the relationship that we discovered through the empirical studies 
% (Section~\ref{subsec:relationship}).
%

% Our goal is to identify a best proxy from the sampled FOVs that best approximates the 
% optimal visual. 
%
Based on the observations in Figure~\ref{fig:pattern_analysis}, where the victim 
token (\textit{clock}, in this case) usually displays a drastically peaking 
distribution while the hallucinating tokens are either noisy or shift monotonically 
with the visual context, \jz{I feel this is something we want to highlight as an observation motivating our method. Maybe we can think of ways to separate it out a little bit.} we propose a \textit{dynamic FOV selection} method to identify 
the top $m$ proxies with largest contextual discrepancy to effectively filter 
the peaking distribution tokens to approximate the unknown optimal visual prior. 
%
Mathematically, we have:
%
\begin{equation}\label{eqn:JSD_filter}
    \tilde{v}^* = \underset{(i,j) \sim \pi(\tilde{v}|v_D)}{\arg\,\max} \; d\left(p_{\theta}(y_t | \tilde{v}_i, x, y_{<t}),  p_{\theta}(y_t | \tilde{v}_j, x, y_{<t})\right),
\end{equation}
%
where $d$ is the Jensen-Shannon divergence (JSD)~\cite{chuang2023dola},
a symmetric metric that measures the difference between two distributions.
%
\begin{equation}\label{eqn:JSD}
    d_{i,j}  = \text{JSD}(p_{\theta}(y_{t} | \tilde{v}_i , x, y_{<t}) \parallel  p_{\theta}(y_t | \tilde{v}_j,  x, y_{<t}))
\end{equation}
%
To take into account the fact that each token may rely on different levels of context 
(e.g., pixel, texture, color, object, scene) to be correctly predicted, we preserve the top 
$m$ pairs of logits distributions of relative largest divergence instead of the 
maximum token in Eqn.~(\ref{eqn:JSD}). 
%
While there is no robustness guarantee for  directly using $\tilde{v}_d$ (or any single heuristic-based visual prior) as a proxy for $v^*$, we could essentially certify the robustness for our proposed dynamic multi-sample FOV selection strategy.
%
Considering the deviation of the grounded visual prior $\tilde{v}_d$ and $v^*$ as a perturbation $\eta$, we provide its robustness certification in Theorem~\ref{theorem:robustness}.
%
% we could certify the robustness of this dynamic multi-sample FOV selection process from 
% distribution $\pi_f(\tilde{v}|v_d)$.

% Assuming Eqn.~(\ref{eqn:JSD}) is an oracle that could effectively select the most appropriate 
% FOV from the samples, we derive the analytical form of the \textit{expected deviation} of our 
% algorithm to predicting the non-hallucinating token.
% %
% Furthermore, we provide upper bounds for normal and exponential distributions in 
% Theorem~\ref{thm:robustness}.
%

\begin{theorem}\label{theorem:robustness}
Let $v^*$ be the optimal visual prior within a neighborhood $\mathcal{N}(v^*, \epsilon)$ %\rv{bounded by radius $\epsilon$.}
bounded by radius $\epsilon$.
%where the deviation in the distribution at $v^*$ compared to any other point $v$ within this neighborhood is bounded by $\Delta g(v^*,v)$. 
%\bo{do you wanna say this neighborhood is bounded by radius $\epsilon$?}
%
Consider a perturbation $\eta = \|\tilde{v}_d - v^*\|$ satisfying $ \epsilon < C_{I_2} \leq \eta \leq C_{I_1}$,
%\rv{$ \epsilon < C_{I_2} \leq \eta \leq C_{I_1}$}, 
%
the expected deviation $\mathbb{E}[g(v^*,v)]$ with $N$ samples from an arbitrary sampling 
distribution $\pi_f(\tilde{v}_d) \in \Omega$ is given by:
%
\begin{small}
    \begin{equation}
        \mathbb{E}[g(v^*,v)] = %\frac{1}{N} \sum_{i=1}^{N}
    \mathbb{E}_{\tilde{v}_i \sim \pi_f(\tilde{v}_i | v_d)}\left[|p_{\theta}(y_t | v^*) - p_{\theta}(y_t | \tilde{v}_i)|\right]
    \end{equation}
\end{small}
%

Therefore, for normal sampling distribution $ \tilde{v}_{\pi_f}=\mathbb{N}(\tilde{v}_d, \sigma)$ and 
exponential sampling distribution $\tilde{v}_{\pi_f}=(1 + \lambda)^n \cdot \tilde{v}_d$, their respective 
upper bounds are:
%
\begin{small}
\begin{align}
    \mathbb{E}[g(v^*,\tilde{v})] &\leq \left(1 - \int_{v^*- \epsilon}^{v^*+\epsilon} \frac{1}{\sigma\sqrt{2\pi}} e^{-\frac{(\tilde{v} - (v^* + \eta))^2}{2\sigma^2}} \, d\tilde{v} \right)^N \leq C_S   \\
    % \mathbb{E}[g(v^*,v)] &\leq \left(1 - \frac{\log\left(\frac{v^* + \epsilon}{v^* - \epsilon}\right)}{\log(1 + \lambda)}\right)^N \leq C_S.
    \mathbb{E}[g(v^*,\tilde{v})] &\leq \left(1 - {\log\left(\frac{v^* + \epsilon}{v^* - \epsilon}\right)}/{\log(1 + \lambda)}\right)^N \leq C_S
\end{align}
\end{small}
%
\end{theorem}
%
The proof of Theorem~\ref{theorem:robustness} is detailed in Appendix~\ref{app:robustness}.
%
%\rv{The constraint $ \epsilon < C_{I_2} \leq \eta \leq C_{I_1}$ on the perturbation is to identify the general case where $\tilde{v}_d$ cannot sufficiently approximate $v^*$ while an effective sample might succeed. The radius $\epsilon$ can be roughly interpreted as a valid range of optimal visual prior to yield the correct prediction (e.g., $[2\tilde{v}_d, 3\tilde{v}_d$] in Figure~\ref{fig:optimal_visual_prior}).} 
The constraint $ \epsilon < C_{I_2} \leq \eta \leq C_{I_1}$ on the perturbation is to identify the general case where $\tilde{v}_d$ cannot sufficiently approximate $v^*$ while an effective sample might succeed. The radius $\epsilon$ can be roughly interpreted as a valid range of optimal visual prior to yield the correct prediction (e.g., $[2\tilde{v}_d, 3\tilde{v}_d$] in Figure~\ref{fig:optimal_visual_prior}).
The robustness of the proposed dynamic multi-sample FOV selection is characterized by the 
upper bound $C_S$, which depends on the detector perturbation $\eta$ and sampling distribution ($\sigma$ 
for normal and $\lambda$ for exponential). 
%
While increasing $N$ and adjusting the distribution parameters can efficiently reduce $C_S$ and enhance the 
robustness against bounded perturbations, %\rv{it's notable that the runtime costs also raise with $N$. Consequently, we set $N=4$ across all our experiments.}
it's notable that the runtime costs also raise with $N$. Consequently, we set $N=4$ across all our experiments.
%
% \rv{Typically, a normal distribution, which concentrated around $\tilde{v}_d$, provides a tighter bound under minimal perturbations, 
% while an exponential distribution, with a more averaged coverage of the sampling space, is preferable when less priors of the task is 
% available.}
Typically, a normal distribution, which concentrated around $\tilde{v}_d$, provides a tighter bound under minimal perturbations, 
while an exponential distribution, with a more averaged coverage of the sampling space, is preferable when less priors of the task is 
available.
%
% \begin{theorem}\label{thm:robustness}
% Let $v^*$ be the optimal visual prior within a neighborhood $\mathcal{N}(v^*, \epsilon)$, 
% where the distribution deviation within this neighborhood is bounded by $\Delta g(v^*,v)$. 
% %
% Consider a perturbation $\eta = \|\tilde{v}_d - v^*\|$ satisfying $\| \mathcal{N}(v^*, 
% \epsilon) \| < C_{I_2} < \eta < C_{I_1}$. The expected deviation with $N$ samples from an 
% arbitrary sampling distribution $\pi_f(\tilde{v}_d) \in \Omega$ is
% %
% {\small
% \begin{equation}
%     \mathbb{E}[g(v^*,v)] = \frac{1}{N} \sum_{i=1}^{N} \mathbb{E}_{\tilde{v}_i \sim \pi_f(\tilde{v}_i | v_d)}\left[|p_{\theta}(y_t | v^*) - p_{\theta}(y_t | \tilde{v}_i)|\right].
% \end{equation}
% }
% %

% Specifically, for normal distribution $\mathbb{N}(\eta, \sigma)$, the upper bound of
% the expected deviation is
% {\small
% \begin{equation}
%     \mathbb{E}[g(v^*,v)] \leq \left(1 - \int_{v^*- \epsilon}^{v^*+\epsilon} \frac{1}{\sigma\sqrt{2\pi}} e^{-\frac{(\tilde{v} - (v^* + \eta))^2}{2\sigma^2}} \, d\tilde{v} \right)^N \leq C_S
% \end{equation}
% }

% and for exponential distribution $(1 + \lambda)^n(v^* + \eta)$, the upper bound becomes
% %
% \begin{equation}
%     \mathbb{E}[g(v^*,v)] \leq \left(1 - {\log\left(\frac{v^* + \epsilon}{v^* - \epsilon}\right)}/{\log(1 + \lambda)}\right)^N \leq C_S
% \end{equation}
% %
% \end{theorem}
% %
% The proof is detailed in appendix~\ref{app:robustness}. While increasing $N$, and adjusting 
% $\sigma$, or $\lambda$ can achieve better robustness certificate $C_S$, the specific choice 
% of the sampling distribution depends on many factors (e.g. perturbation magnitude, LVLM 
% backbone, tasks). 
% %
% Typically, a normal distribution provides a tighter bound under minimal perturbations, while 
% an even-sized exponential distribution is preferable when less priors of the task is 
% available.
% %

After obtaining the top $m$ logits distribution pairs, we contrast them to amplify the 
information of the expert visual priors in each pair while attenuating other noisy 
hallucination patterns. 
%
This provides more precise and distinguished signals specific to each FOV for 
subsequent decoding~\cite{li2022contrastive}. 
%
Specifically, for each pair of FOVs $(\tilde{v}_i, \tilde{v}_j)$, the model generates 
two distinct output distributions conditioned on each FOV respectively. 
%
Then the redistributed logits distribution $p_{\text{FOV}}$ is formulated as:
%
\begin{align}\label{eqn:p_fov}
p_{\text{FOV}} (y_t | \tilde{v}_e, \tilde{v}_a, x, y_{<t}) &= \sigma \Big[ (1 + \alpha) \text{logit}_{\theta} (y_t | \tilde{v}_e, x, y_{<t}) \nonumber \\
\quad - \alpha & \text{logit}_{\theta} (y | \tilde{v}_a, x, y_{<t}) \Big]
\end{align}
%
where $y_t \in \mathcal{V}_{\text{head}}(y_{<t})$, and $\tilde{v}_e$, $\tilde{v}_a$ 
denote the expert and amateur distribution of each pair respectively.
%
$\sigma$ here represents the softmax function, and $\alpha$ is the amplification factor 
where larger $\alpha$ value indicates a stronger amplification of the differences 
between the distribution pair 
($\alpha = 0$ simplifies Eqn.~(\ref{eqn:p_fov}) to regular decoding without contrast). 
%

To preserve the plausibility and linguistic quality after contrasting, we involve the 
adaptive plausibility set~\cite{li2022contrastive} $\mathcal{V}_{\text{head}}$ as a 
constraint which contingents upon the confidence level associated with the expert 
output distribution:
%
\begin{align}
\mathcal{V}_{\text{head}} (y_{<t}) & = \{ y_t \in \mathcal{V} :\nonumber \label{eq:adaptive_plausibility_constraint}\\
p_{\theta}(y_t | v_e,   x, y_{<t}) \geq & \beta \max_{w} p_{\theta}(w | v_e, x, y_{<t}) \}, \\
 p_{\text{FoV}} (y_t | v_e, v_a, x) = & 0, \text{ if }  y_t \notin V_{\text{head}} (y_{<t}) \nonumber
\end{align}
%
The benefit of this adaptive plausibility constraint is that it excludes two singular 
cases after contrast: (1) false positive: an implausible token with an extremely low 
score may be rewarded with a high score after contrast due to their noisy probability 
range across different FOVs (e.g., \textit{book} in Figure~\ref{fig:optimal_visual_prior}); 
(2) false negative: for plausible and obvious tokens across different levels of context 
(e.g. \textit{beach} in Figure~\ref{fig:optimal_visual_prior}), their output probability 
would maintain high and thus result in low scores after contrast. 
%
Therefore, the adaptive plausibility constraint effectively excludes these implausible 
tokens while enforcing the model to still select those high-score plausible tokens 
after contrast.

% Next, we propose to contrast the distributions of visual priors in each FoV to identify the FoV that involve the peaking context. 

However, unlike existing uni-modal contrastive methods that indicate expert and amateur 
distributions by assuming the final-layer~\cite{chuang2023dola, gera2023benefits} or 
the context-aware input~\cite{shi2023trusting} contains more factual knowledge, we 
argue that defining the expert distribution among a pair of FOVs is non-trivial. 
%
For example, the optimal visual prior usually resides midway among FOVs, making either 
overflowing or insufficient context result in hallucination (Figure~\ref{fig:optimal_visual_prior}). 
%
Therefore, instead of defining such distinct roles, for each pair of logit distributions, we propose to contrast them bi-directionally which consists of both \textit{positive contrast} (larger over smaller-sized FOV) and \textit{negative contrast} (smaller over larger-sized FOV) to preserve the completeness of FOV representations (as shown in Figure~\ref{fig:halc_overview}). Eventually, this process results in $2*m$ candidate tokens, and we leave the following matching-based beam search algorithm to further select them from a global perspective. 
%

% To conclude, the purposes of our proposed dynamic contrasting are
% (1) ensuring the peaking pattern of the victim object token be selected by JSD while 
% attenuating other noisy hallucination patterns; 
% and (2) amplifying the information of the visual priors in each retrieved FoV 
% to provide more distinguished and precise signals for subsequent decoding.
% decoding methods contrast logits distributions
% While recent popular contrastive 
% decoding methods contrast logits distributions between a static expert and amateur~\cite{chuang2023dola, shi2023trusting, gera2023benefits} and assume the final-layer or context-aware input contains more factual knowledge. However, given our analysis in Section~\ref{subsec:relationship} that retrieving 



% inspired by recent studies on contrastive 
% decoding~\cite{chuang2023dola, shi2023trusting, gera2023benefits}, where less hallucinating
% responses are generated through contrasting logits distributions between expert and amateur 
% layers, we propose to contrast distributions from visual priors among different pairs of FoVs.




%
% Specifically, for each located region returned by visual grounding, we generate additional 
% smaller and larger regions by varying the FOVs, resulting in $n$ cropped images in total, 
% where $n$ is an hyperparameter of the algorithm.
%
% An example of these regions is the $[I_S, I_D, I_L]$ in Figure~\ref{fig:halc_overview}, 
% where $I_D$ is the grounded region, with $I_S$ and $I_L$ being the regions with smaller 
% and larger FOV respectively.
%

%All the cropped regions, as well as the current response (without the new token generated from the conventional decoding), are then fed back into the LVLM, where $n$ corresponding logits distributions are obtained.
%
% Here, we think of visual priors with different FOVs in analogy to the different layers in the
% existing textual contrastive decoding algorithms.
% %
% However, we don't have a clear definition of expert or amateur layer, which is a prerequisite 
% for any type of contrast in existing works.
% %

% Alternatively, instead of defining such distinct roles, we propose to compute bi-directional
% (both larger FOV over smaller FOV and small over large) pair-wise contrast on all the logits 
% distributions, meaning that $n(n-1)$ pairs of contrasted distributions will be obtained.
% %
% Among these pairs, top $m$ are chosen based on the largest Jensen-Shannon Divergence (JSD)
% where $m$ is also an hyperparameter of the algorithm.
% %

% Finally, the $m$ corresponding contrasted distributions will be used to provide candidates
% for the corrected token.
% %
% As showed in Figure~\ref{fig:halc_overview}, we have $m=4$ contrasted distributions outputting
% "clock", "clock", "wood", and "surfboard" as the candidates.
% %



\subsection{Matching-Based Beam Search}\label{subsec:beam_search}
\setlength{\textfloatsep}{12pt}
\begin{algorithm}[t!]\label{algo:halc_decoding}
\caption{HALC Decoding}
\begin{algorithmic}[1]
% \REQUIRE LVLM $M_{\theta}^{\text{LVLM}}$; text query $x$; original visual input $v$; 
% visual grounding detector $\mathcal{G}_{d}$; an arbitrary FOV sampling distribution 
% $\pi_{f}$; FOV sample size $n$; beam size $k$; JSD filter buffer $m$; 
    \REQUIRE LVLM $M_{\theta}^{\text{LVLM}}$, text query $x$, image query $v$, 
    grounding detector $\mathcal{G}_{d}$, FOV sampling distribution 
    $\pi_{f}$, FOV sample size $n$, beam size $k$, JSD filter buffer $m$. 
    \OUTPUT Model response $y_{\text{new}}$.
    % \Ensure a validated target response $s_T$ is obtained.
    \REPEAT
        \FOR{$b = 1$ to beam size $k$}
        \STATE $M_{\theta}^{\text{LVLM}}$ decoding, obtain current word $w_i^b$.
        \IF{$w_i^b \in \{\text{existence}, \text{attribute}, \text{relationship}\}$}
        \STATE Retrieve visual groundings $v_d^b \leftarrow \mathcal{G}_{d}(w_i^b, v)$
        \ENDIF
        \IF{$v_d^b \neq \{\varnothing\}$}
        \STATE Sample $n$ FOV w.r.t. $\pi_{f}(\tilde{v}^b|v_d^b)$ \COMMENT{\S\ref{para:logits_redistribution}, Eqn.~(\ref{eqn:FoV_sample})}
        \ELSE 
        % \STATE Randomly sample $n$ FOVs w.r.t. unconditional $\pi_{FoV}(\tilde{v}^b)$ or normal $\mathcal{N}(\tilde{v}^b)$ distribution
        \STATE Randomly sample $n$ FOVs w.r.t. $\pi_{f}(\tilde{v}^b)$ 
        %$\{\tilde{v}_1, \tilde{v}_2, \ldots, \tilde{v}_n\} \sim \pi_{FoV}(\tilde{v} | v_d)$ %, \quad \pi_{FoV} \in \Omega$
        \ENDIF
        \STATE Calculate pair-wise JSD $d_{i \neq j}$
        \COMMENT{\S\ref{para:logits_redistribution}, Eqn.~(\ref{eqn:JSD})}
        \STATE Select top-$m$ candidate pairs
        \COMMENT{\S\ref{para:logits_redistribution}, Eqn.~(\ref{eqn:JSD_filter})}
        \FOR{$i = 1$ to $m$}
        \STATE Apply bi-directional contrast $(p_{\tilde{v}_i/ \tilde{v}_j},p_{\tilde{v}_j/ \tilde{v}_i})$, 
        \STATE get a pair of redistributed logits
        \COMMENT{\S\ref{para:logits_redistribution}, Eqn.~(\ref{eqn:p_fov})}
        \ENDFOR
        \COMMENT{$y_{\text{new}}^b$ with $2m$ candidates obtained}
        \ENDFOR 
        \STATE Select top $k$ candidate responses 
        \COMMENT{\S\ref{subsec:beam_search}, Eqn.~(\ref{eqn:matching_score})}
        \IF{$v_d^b \neq \{\varnothing\}$ \AND $y_{\text{new}}^b=w_i^b$}
        \STATE $y_{\text{new}}^b$ $\leftarrow$ [IDK]
        \COMMENT{$w^b_i$ is hallucinating, but no correct token was found}
        \ENDIF
        \STATE $w_i^b \leftarrow y_{\text{new}}^b$
        \COMMENT{Hallucinating token $w_i^b$ corrected}
    \UNTIL{each beam has terminated}
\end{algorithmic}
\end{algorithm}
%
To further optimize on choosing the best non-hallucinating token from the adaptive 
focal-contrast grounding, as well as making sure the response at each step aligns well 
with the original visual input, we propose \textit{matching-based beam search} to guide 
the text generation process in a global sense.
%
% On a high level, similarity-based beam search utilizes the cosine similarity between the 
% currently generated text (that is still being generated) and the original input visual prior as 
% the beam score to select the most appropriate caption at the end.
%

Similar to the standardized beam search methods~\cite{anderson2016guided}, 
we start with an initial token that serves as the root of the search tree, while keeping 
the top $k$ probable sequences, where $k$ is an hyperparameter of the algorithm.
% %
% When the beam size $k=1$, the algorithm is essentially a matching-based greedy search,
% which is a special case when shorter runtime is hugely preferred.
% %
%
For %each step in the text generation, or in other words, 
each token in the decoding process, as illustrated in 
Section~\ref{subsec:focal_contrast_grounding}, we have $2m$ logits distributions
from the top focal-contrast pairs, resulting in $2mk$ response sequences in the 
search tree.
%
Different from existing beam score designs~\cite{borgeaud2019leveraging}, we focus on 
using the cosine similarity as the beam score, selecting $k$ distinct sequences from the 
$2m \cdot k$ candidates to maintain diversity.
%
\begin{align}
S = \text{argmax}_{y_t} &(\text{score}(y_{\leq t}, v)) \label{eqn:matching_score} \\
\text{s.t.} \hspace{0.1in} \forall y_{\leq t} \in S, i \neq &j: s_i \neq s_j, |S| \leq 2m \cdot k \nonumber
\end{align}
%
where $S$ is the set of $2m \cdot k$ candidate responses.
%
In practice, we employ bootstrapping language-image pre-training (BLIP)
~\cite{li2022blip} %contrastive language-image pretraining (CLIP)~\cite{radford2021learning}
for both text and image encoding when computing the similarity scores. %., then we select the sequence with highest image-text similarity
%score as the final output.
%
The complete algorithm of HALC summarizing all the components discussed in this section 
is showed in Algorithm~\ref{algo:halc_decoding}.
%

